Language as an Abstraction for Hierarchical Deep Reinforcement Learning

Solving complex, temporally-extended tasks is a long-standing problem in reinforcement learning (RL). We hypothesize that one critical element of solving such problems is the notion of compositionality. With the ability to learn concepts and sub-skills that can be composed to solve longer tasks, i.e. hierarchical RL, we can acquire temporally-extended behaviors. However, acquiring effective yet general abstractions for hierarchical RL is remarkably challenging. In this paper, we propose to use language as the abstraction, as it provides unique compositional structure, enabling fast learning and combinatorial generalization, while retaining tremendous flexibility, making it suitable for a variety of problems. Our approach learns an instruction-following low-level policy and a high-level policy that can reuse abstractions across tasks, in essence, permitting agents to reason using structured language. To study compositional task learning, we introduce an open-source object interaction environment built using the MuJoCo physics engine and the CLEVR engine. We find that, using our approach, agents can learn to solve to diverse, temporally-extended tasks such as object sorting and multi-object rearrangement, including from raw pixel observations. Our analysis reveals that the compositional nature of language is critical for learning diverse sub-skills and systematically generalizing to new sub-skills in comparison to non-compositional abstractions that use the same supervision.

==> section_intro.tex <==

\section{Introduction}
\label{intro}

Deep reinforcement learning has seen remarkable advancements in recent times. For example, reinforcement learning agents can solve difficult continuous control tasks~\citep{schulman2015high,lillicrap2015continuous,gu2017deep,heess2017emergence} and achieve impressive
performance on many challenging games such as Atari games \cite{dqn} and Go \cite{alphago}. The generality of reinforcement learning makes it an ideal framework for optimizing a wide range of sequential decision-making problems. However, many challenges remain for applications of reinforcement learning.
Questions such as long-horizon planning or receiving instructions from a human in the loop are still open problems. In this work, we are interested in building intelligent agents that are able to learn complex, temporally extended skills (e.g. arranging multiple objects) and, at the same time, reason using language.

One approach that attempts to address the temporally extended nature of tasks is {\it hierarchical reinforcement learning} (HRL) \cite{dayan1993feudal, parr1998reinforcement}.
In standard settings of HRL, the agents leverage a hierarchy of policies with varying levels of temporal and behavioral abstractions, where the high-level policy achieves long-horizon tasks 
by controlling the low-level policies,
which focus on more short-term tasks such as moving in a specific direction. 

While, in principle, HRL is a promising framework for solving temporally extended tasks, it is highly non-trivial to apply it in practice.
One challenge of applying HRL is to choose the appropriate abstraction. Hard-coded abstractions often lack modeling flexibility and are task-specific~\citep{sutton1999between,konidaris2007building,heess2016learning, deepLoco}, while learned abstractions require carefully-tuned regularization~\citep{bacon2017option,harb2017waiting}.
One possible solution is to have the higher-level policy generate a goal state
and have the low-level policy try to reach that goal state. Intuitively, a goal state can be seen as an instruction to the low-level policy. 
So far, most works in goal-conditioned reinforcement learning have used simple goal representations such as points in the state space, which does not scale well into high dimensional state space~\citep{uvfa,her}. For instance, in the visual domain, generating high fidelity images is still an area of active research. 

In contrast, language is a flexible representation for transferring a variety of ideas and intentions with minimal assumptions about the problem setting, while its  compositional nature makes it a powerful abstraction for transferring knowledge and instructions~\citep{grice1975logic,mordatch2018emergence}.
In this work, we propose to use language as the interface between high- and low-level policies in hierarchical reinforcement learning.
With a low-level policy that follows instructions, the high-level policy can produce actions in the space of language, giving us a number of appealing benefits.
First, the low-level policy can be re-used for different high-level objectives without retraining. Second, the high-level policies are human interpretable as the action space consists of instructions in language; the low-level policy that understands language instruction also allows human to communicate with the agent, making it easier to recognize and diagnose failures.
Finally, studies have also suggested that humans use language as an abstraction for reasoning and planning \cite{language_ang_thought, piantadosi2012bootstrapping}. In fact, the majority of knowledge learning and skill acquisition we do are through languages throughout our life.

While language is an appealing choice as the abstraction for HRL, training a low-level policy that is capable of following language instruction is a non-trivial problem as it involves learning from binary reward signals that indicate whether or not the instruction was completed. To address this problem, we extend and generalize previous work on goal relabeling to the space of language goals, allowing the agent to learn from many language instructions at once.
We evaluate on a new interactive environment that consists of procedurally-generated scenes of objects that are paired with programatically-generated language descriptions. The low-level policy's objective is to manipulate the objects in the scene such that a description or statement is satisfied by the arrangement of objects in the scene. On high-level object reconfiguration and sorting tasks, we find that language abstractions and hindsight instruction relabeling are critical for learning a wide variety of these temporally-extended skills.

In summary,
the main contribution of our work is three-fold:
\begin{enumerate}
     \item a framework for incorporating language abstractions into hierarchical RL, with which we find that the structure and flexibility of language enables agents to solve a variety of long-horizon control problems
     \item an algorithm for effectively training a multi-task reinforcement learning agent to complete language-based instructions through {\it hindsight instruction relabeling}.
     \item an open-source interactive continuous control environment integrated with language tasks inspired by the CLEVR dataset \citep{clevr}, built on MuJoCo physics simulator~\citep{todorov2012mujoco}.
\end{enumerate}
